Theory and Applications of Kernel Stein's Method on Riemannian Manifolds

Distributional comparison is a fundamental problem in statistical data analysis with numerous applications in a variety of scientific and engineering fields. Numerous methods exist for distributional comparison but kernel Stein's method has gained significant popularity in recent times. In this paper, we first present a novel mathematically rigorous and consistent generalization of the Stein operator to Riemannian manifolds. Then we show that the kernel Stein discrepancy (KSD) defined via this operator is nearly as strong as the KSD in the Euclidean setting in terms of distinguishing the target distributions from the reference. We investigate the asymptotic properties of the minimum kernel Stein discrepancy estimator (MKSDE), apply it to goodness-of-fit testing, and compare it to the maximum likelihood estimator (MLE) experimentally. We present several examples of our theory applied to commonly encountered Riemannian manifolds in practice namely, the n-sphere, the Grassmann, Stiefel, the manifold of symmetric positive definite matrices and other Riemannian homogeneous spaces. On the aforementioned manifolds, we consider a variety of distributions with intractable normalization constants and derive closed form expressions for the KSD and MKSDE.

==> KSD-EM_material/KSD-EM.tex <==

\subsubsection{The KSD-EM Algorithm}\label{KSD-EM}

The classical EM algorithm is used to estimate the parameter \(\theta\) of a probabilistic model \(x\sim p(x,y|\theta)\) with a latent variable $y$. With only samples of $x$, the MLE may marginalize the model as
$p_X(x;\theta)=\int p(x,y) d z$, but such quantity is often intractable since $y$ is unobserved, as in the probabilistic principal geodesic analysis (PPGA) technique \cite{zhang2014bayesian,zhang2013probabilistic,zhang2019mixture} on Riemannian manifolds, or the estimation of mixture of distributions \cite{???}. 

We denote the statistical model by $p(x,y|\theta)$, where $\boldsymbol{x}$ is the observed samples and $y$ is the latent variable. The EM algorithm generates an iterate $\theta_t$ of $\theta$ by "E-step" and "M-step". The E-step compute the log-likelihood $Q(\theta|\boldsymbol{x},\theta_{t})$ marginalized over $y\sim p(y|\boldsymbol{x},\theta_t) $, then the M-step maximizes $Q(\theta|
\theta_t)$ to get the next iteration, i.e., 
\[
\textbf{E-step:}\ \ 
Q(\theta|\theta_t):= \mathbb{E}_{y\sim p(y|\boldsymbol{x},\theta_t) } [\log p(y,\boldsymbol{x}|\theta)]\qquad
\textbf{M-step:}\ \ \theta_{t+1}:=\argmax Q(\theta|\theta_t).
\]

The EM-algorithm is an alternating minimization algorithm \cite[\S 1.6.3 \& \S 8.1]{amari2016information}, which alternately minimizes the KL-divergence between two statistical manifolds:
\begin{equation}\label{D&M}
\mathcal{M}:= \{ p(x,y|\theta) \},\quad
\mathcal{D}:=\{\Bar{q}(x,y):=\Bar{q}_X(x)q(y|x): q(y|x) \text{ is arbitrary} \},
\end{equation}
where $\Bar{q}_X(x):=n^{-1}\sum_{i=1}^n \delta_{x_i}(x) $ is the empirical distribution of the observed samples $\boldsymbol{x}$. Suppose we fix $\theta=\theta_0$, then the point on statistical manifold $\mathcal{M}$ will fix at $p(x,y|\theta^t)$. As shown in Fig.\ref{fig:GeoEM}, the E-step(E-projection) will minimizes the KL divergence between the point $p(x,y|\theta^t)\in\mathcal{M}$ and the manifold $\mathcal{D}$, and get the minimizer $\eta_1:=\Bar{q}_X(x)\cdot p(y|x,\theta_0) $. Next, the M-step(M-projection) minimizes the KL-divergence between the point $\eta_1\in\mathcal{D} $ and the manifold $\mathcal{M}$, and get the minimizer $p(x,y|\theta_1)\in\mathcal{M}$. We repeat this process and get the iteration $\theta_t$. We refer the readers to \cite[\S 8.1]{amari2016information} for the detailed illustration.

Note that the M-step maximizes a marginalized log-likelihood, thus one may encounter difficulty as the log-likelihood $\log p(x,y|\theta)$ is dependent of the normalizing constant, e.g., the mixture of von-Mises fisher on sphere \cite{???}. To handle such situations, we may replace the log-likelihood with the weighted KSD from (\ref{wMKSDE-discreted}) and cope with the issue of the intractable normalizing constants. Suppose random variables $x$ and $y$ take values in $\mathcal{X}$ and $\mathcal{Y}$. We adopt the notations $\mathcal{S}_p$, $\Tilde{\mathcal{S}}_p$, $k$, $\Tilde{k}$, $k_p$, $\tilde{k}_p$ and $\mathcal{K}_p$ from \S\ref{KSD-Product}. The \emph{KSD-EM algorithm} takes following two steps:
\begin{equation}\label{KSD-EM-Eq}
\begin{aligned}
\textbf{E-step:}\qquad &Q_{\wksd}(\theta|\theta_t):= \mathbb{E}_{y,y'\sim p(y|x,\theta_t) }\left[ \mathcal{K}_{p(x,y|\theta)}(\boldsymbol{x},\boldsymbol{x'},y,y') \right],\\
\textbf{M-step:}\qquad &\theta_{t+1}:=\argmin Q_{\wksd}(\theta|\theta_t),
\end{aligned}
\end{equation}
where $\mathcal{K}_{p(x,y|\theta)}(\boldsymbol{x},\boldsymbol{x'},y,y'):=n^{-2}\sum_{i,j} \mathcal{K}_{p(x,y|\theta)}(x_i,x_j,y,y')$.

\begin{figure}
    \centering
\includegraphics[width=6cm]{41884_2022_80_Fig1_HTML.png}
    \caption{Geometric perspective of the EM algorithm \cite[Fig.1]{hino2024geometry} }
    \label{fig:GeoEM}
\end{figure}

\begin{algorithm}
\caption{KSD-EM algorithm
}    

\textbf{Input}: population \(\boldsymbol{x}\sim q\);  initial value $\theta_0$; iteration count $t=0$; error tolerance $\epsilon$.

\textbf{while} {$|Q_{\wksd}(\theta_t|\theta_{t-1})-Q_{\wksd}(\theta_{t-1}|\theta_{t-2})|>\epsilon$}

\Indp 
1. Sample $y_1,\dots,y_n\sim \omega$.

2. Compute $\theta_{t+1}:=\argmin_\theta Q_{\wksd}(\theta|\theta_t)$ numerically or analytically.

3. $t\leftarrow t+1$.

\Indm

\textbf{end while}

\textbf{Output:} $\theta^t$.
\end{algorithm}

Akin to the EM algorithm, the KSD-EM algorithm is also an alternating minimization algorithm. However, it minimizes the KSD instead of the KL-divergence between the statistical manifolds $\mathcal{M}$ and $\mathcal{D}$ in (\ref{D&M}). The KSD between $\mathcal{M}$ and $\mathcal{D}$ is 
\[
\ksd(p(x,y|\theta),\Bar{q}_X(x)q(y|\boldsymbol{x},\theta))=\frac{1}{n^2} \sum_{i,j=1}^n\iint \mathcal{K}_{p(x,y|\theta)} (x_i,x_j,y,y') q(y|x_i)q(y'|x_j)  \nu(dy) \nu(dy),
\]
for $p(x,y|\theta)\in\mathcal{M}$ and $\Bar{q}_X(x)q(y|x)\in\mathcal{D}$. To perform the E-projection, we fix $\theta=\theta_0$, i.e., fix the point on $\mathcal{M}$ at $p(x,y|\theta_0)$, and then search for the minimizer $\eta_1\in\mathcal{D}$ that minimizes the KSD between $p(x,y|\theta_0)$ and $\mathcal{D}$. In fact, we have

\begin{theorem}\label{KSD-EM-Estep} $\eta_1:=\Bar{q}_X(x)p(y|x,\theta_0)\in\mathcal{D}$ minimizes the KSD between $p(x,y|\theta_0)\in\mathcal{M}$ and $\mathcal{D}$, i.e.,
\[\eta_1=\argmin_{\eta\in\mathcal{D}}\ksd(p(x,y|\theta_0),\eta).
\]
\end{theorem}
\begin{proof} The proof is included in appendix \ref{Proof-KSD-EM-Estep}.
\end{proof}

We then perform the M-projection. We fix $\eta$ at $\eta_1:=\Bar{q}_X(x)p(y|x,\theta_0)$ and search for $\theta_1\in\Theta$ such that
\[
\begin{aligned}
\theta_1&=\argmin_{\theta\in\Theta} \ksd(p(x,y|\theta),\bar{q}_X(x)p(y|x,\theta_0))\\
&=\argmin_{\theta\in\Theta} \iint \frac{1}{n^2}\sum_{i,j=1}^n \mathcal{K}_{p(x,y|\theta)}(x_i,x_j,y,y') p(y|x_i,\theta_0) p(y'|x_j,\theta_0) \nu(dy) \nu(d y'),
\end{aligned}
\]
which is exactly the M-step in (\ref{KSD-EM-Eq}). We repeat the E-step and M-step introduced in (\ref{KSD-EM-Eq}) to get the iterate $\theta_n$.


\begin{theorem}  The KSD-EM algorithm converges

\end{theorem}




==> content/0MainText.tex <==
\input{content/Introduction}
\input{content/Background}
\input{content/Main_Results}
\input{content/MKSDE}
\input{content/Examples}
\input{content/Experiments}

\section*{Acknowledgements}
This research was in part funded by the NIH NINDS and NIA grant RO1NS121099 to Vemuri.

\bibliographystyle{plain} 
\bibliography{reference}

==> content/Hyperbolic.tex <==

\subsection{Hyperbolic Space \texorpdfstring{$\mathbb{H}^N$}{HN}}

There are multiple ways to define the Hyperbolic space. For computational simplicity, we adopt the following \emph{Hyperboloid model}. 

The space $\mathbb{H}^N:=\{x:=\genfrac(){0pt}{2}{s}{t} \in\mathbb{R}^{N+1}: \Vert s\Vert^2+1=t^2, s\in\mathbb{R}^N, t>0\}$, inheriting the differential structure from $\mathbb{R}^{N+1}$ as a subspace, is a smooth manifold. Let
\[
J:=
\begin{pmatrix}
I_N & 0\\
0 &  -1
\end{pmatrix}\in\mathbb{R}^{(N+1)\times(N+1)}
\]
The \emph{Minkowski bilinear form}, a.k.a. \emph{Lorentz inner product} on $\mathbb{R}^{N+1}$, defined as $L(x,y)=x^\top J y$, $x,y\in\mathbb{R}^{N+1}$ is positive definite when being restricted on the tangent space of $\mathbb{H}^N$, thus forms a Riemannian metric tensor on $\mathbb{H}^N$. Accordingly, $(\mathbb{H}^N,L)$, which is a Riemannian manifold, is said to be the \emph{Hyperbolic space}. The distance function on $\mathbb{H}^N$ is given by $d(x,y)=\cosh^{-1} (-L(x,y)).$ The Riemannian exponential map and logarithm map are given by
\[
\Exp_x(v)=\cosh(|v|)x+\frac{\sinh(|v|)}{|v|} v,\quad \Log_x(y)=\frac{d(x,y)}{\sinh(d(x,y))}(y+L(x,y) x),\quad x,y\in\mathbb{H}^N, v\in T_x\mathbb{H}^N.
\]

The \emph{Lorentz group} $\Or(N,1)$ is defined as $\Or(N,1):=\{A^\top\in\GL(N+1): A^\top J A=J\}$, and further the special subgroup $\SO(N,1)$ is defined as $\SO(N,1):=\{A\in\Or(N,1): \det(A)=1\}$. Let $\SO_0(N,1)$ be the connected component of $\SO(N,1)$ that contains the identity. It is known \cite[Prop. 2.11]{gallier2011notes} that $\SO_0(N,1)$ acts transitively on $\mathbb{H}^N$, where the isometry $\Psi_A$ corresponding to each $A\in\SO_0(N,1)$ is given by $\Psi_A(x)=A x$, $x\in\mathbb{H}^N$. In addition, the Lie algebra $\mathfrak{so}(N,1)$ of $\SO_0(N,1)$ is \cite[\S 5.5]{gallier2011notes} satisfies $\mathfrak{so}(N,1):=\mathfrak{p}\oplus\mathfrak{l}$, where
\[
\mathfrak{p}:=
\left\{ \begin{pmatrix}
    B & 0\\
    0^\top & 0
\end{pmatrix} : B\in \mathbb{R}^{N\times N}, B^\top=-B
\right\},\quad \mathfrak{l}:=
\left\{ \begin{pmatrix}
    0 & u\\
    u^\top & 0
\end{pmatrix} : u\in\mathbb{R}^N
\right\}.
\]
Therefore, we choose
\begin{equation}\label{HN-basis}
B_{i j}:=\begin{pmatrix}
E_{i j} & 0\\
0^\top & 0
\end{pmatrix},\quad U_i=\frac{\sqrt{2}}{2}\begin{pmatrix}
    0 & e_i\\
    e^\top_i & 0
\end{pmatrix},\quad 1\leq i,j\leq N,
\end{equation}
as the basis of $\mathfrak{p}$ and $\mathfrak{l}$ respectively. Clearly, for $E\in\mathfrak{so}(N,1)$, the corresponding killing field is given by $Ex, x\in\mathbb{H}^N$. By proposition \ref{kernel-universal}, the kernel we choose is
\begin{equation}\label{HN-kernel}
    k(x_1,x_2)= \exp(-\frac{\tau}{2}\Vert x_1-x_2\Vert^2)=\exp\left( -\frac{\tau}{2}\big(\Vert s_1-s_2\Vert^2+ (t_1-t_2)^2\big)\right) 
\end{equation}
since $x_1=\genfrac(){0pt}{2}{s_1}{t_1} $ and $x_2=\genfrac(){0pt}{2}{s_2}{t_2} $.


\begin{theorem}\label{HN-kp}Given basis in Eq. (\ref{HN-basis}) and kernel function in Eq. (\ref{HN-kernel}), the $k_p$ function is 
\begin{equation}\label{Hyper-kp-Form} 
\begin{aligned}
k_p(x_1,x_2)
&=
s_1^\top(\nabla_{s_2}\log p-\tau(s_2-s_1))\cdot s_2^\top(\nabla_{s_1}\log p-\tau(s_1-s_2)) k\\
&+\frac{1}{4}[t_1((\nabla_{s_2}\log p-\tau(s_2-s_1)))+(\nabla_{t_2}\log p-\tau(t_2-t_1))s_1]^\top\\
&\cdot
[t_2(\nabla_{s_1}\log p-\tau(s_1-s_2))+(\nabla_{t_1}\log p-\tau(t_1-t_2))s_2]\\
&+ \frac{\tau N}{2} x_2^\top x_1 k.
\end{aligned}
\end{equation}
Here $\nabla_s\log p\in \mathbb{R}^N$ is the first $N$ components of $\nabla_x \log p\in\mathbb{R}^{N+1}$ and $\nabla_t\log p\in\mathbb{R}$ is the last component of $\nabla_x \log p\in\mathbb{R}^{N+1}$.
\end{theorem}
\begin{proof} The proof is included in appendix \ref{Proof-HN-kp}.    
\end{proof}




==> content/Steins_lemma.tex <==

The above theorem, leads to a generalization of the classical Stein's lemma \cite[Lem. 2.1]{ross2011fundamentals}. Prior to stating this generalization, we remind the readers with the statement of the classical Stein's lemma: For a real-valued random variable $W$, $W$ follows Gaussian distribution $N(\Bar{x},\sigma^2)$, $\Bar{x}\in\mathbb{R}$, $\sigma>0$, if and only if $\mathbb{E}[\sigma^2 f'(W)+(\Bar{x}-W)f(W)]=0$ for all absolutely continuous function $f$ such that $\mathbb{E}[|f'(W)|]<+\infty$. Using theorem \ref{KSDCharacterization}, we can establish a similar theorem for the Riemannian Gaussian distribution $\phi(x)\propto \exp\left(-\frac{\rho^2(x,\Bar{x})}{2\sigma^2}\right) $, $\Bar{x}\in M$, $\sigma>0$ on the Riemannian manifold $M$.

\begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black,title=Stein's Lemma on Riemannian Manifolds]
\begin{corollary} Let $M$ be a complete Riemannian manifold and $\Log$ be its Riemannian logarithm map. Suppose $W$ is a $M$-valued random variable with locally Lipschitz continuous density $\omega$. Suppose we replace the $p$ and $q$ in Thm. \ref{KSDCharacterization} with $\omega$ and Gaussian density $\phi(x)\propto\exp\left(-\frac{\rho^2(x,\Bar{x})}{2\sigma^2}\right)$,
further that $\sqrt{\kappa(x,x)}|D^l|$, $g(D^l, \Log_x(\Bar{x}))$, $g(D^l,\nabla\log \omega)$, $\sqrt{\kappa_\phi(x,x)}$, $\sqrt{\kappa_\omega(x,x)}$ are $\phi$ and $\omega$-integrable, then
\[
\omega=\phi \iff \mathbb{E}[ \sigma^2 D^l f(W)+ g(D^l, \Log_W(\Bar{x})) f(W) ]= 0,\quad 1\leq \forall l\leq m,\ \forall f\in\mathcal{H}^m_\kappa.
\]
\end{corollary}
\end{tcolorbox}


==> draft.tex <==
%%% MKSDE for Stiefel

Note that the first quadratic term is the only part of  $k_p$ function in (\ref{kp-Stiefel}) and (\ref{kp-Stiefel-RBF}) that is dependent on the distribution $p$ and thus on its parameter $\theta$. First, let us set $\Pi_X:=\nabla^\mathbb{R}_X\log p$, and rewrite (\ref{kp-Stiefel}) into
\[
\begin{aligned}
\frac{k_p(X,Y)}{k(X,Y)}
&=\tr[\mathscr{A}( (\Pi_X+\nabla^{\mathbb{R}}_X \log k) X^\top)^\top \mathscr{A}((\Pi_Y+\nabla^\mathbb{R}_Y \log k) Y^\top) ] +C(X,Y)
\end{aligned}
\]
where $C(X,Y)$ denotes the rest of the terms that are independent of $p$. We split the term of trace into
\[
\begin{aligned}
&\tr[\mathscr{A}(\Pi_X X^\top)^\top \mathscr{A}(\Pi_Y Y^\top) ]+ \tr[\mathscr{A}( \nabla^{\mathbb{R}}_X \log k X^\top)^\top \mathscr{A}(\Pi_Y Y^\top) ]+\tr[\mathscr{A}(\Pi_X X^\top)^\top \mathscr{A}( \nabla^{\mathbb{R}}_X \log k Y^\top) ]\\
=& \underbrace{\frac{1}{2} \tr[X \Pi_X^\top \Pi_Y Y^\top  ]}_{(I)}-\underbrace{\frac{1}{2}\tr[\Pi_X X^\top \Pi_Y Y^\top]}_{(II)}+\underbrace{\tr[ \Pi_Y^\top \mathscr{A}( \nabla^{\mathbb{R}}_X \log k X^\top) Y ]}_{(III)} + \underbrace{\tr[ \Pi_X^\top \mathscr{A}( \nabla^{\mathbb{R}}_Y \log k Y^\top) X ]}_{(IV)},
\end{aligned}
\]
where we combine the terms independent of $p$ into $C$. Note that the second-order terms equal
\[
\begin{aligned}
(I) &=\frac{1}{2}[(X\otimes I_N) \vectz(\Pi_X)]^\top [(Y\otimes I_N)\vectz(\Pi_Y)]=\frac{1}{2}\vectz(\Pi_X)^\top(X^\top Y\otimes I_N) \vectz(\Pi_Y),\\
(II)&=\frac{1}{2} \vectz[X\Pi_X^\top Y]^\top \vectz(\Pi_Y)=\frac{1}{2} \vectz(\Pi_X)^\top (X^\top\otimes Y) S_{N,r} \vectz(\Pi_Y).
\end{aligned}
\]
The first-order terms equal
\[
\begin{aligned}
  (III)&= \vectz(\mathscr{A}( \nabla^{\mathbb{R}}_X \log k X^\top) Y)^\top \vectz(\Pi_Y),\\
  (IV)&=  \vectz(\mathscr{A}( \nabla^{\mathbb{R}}_Y \log k Y^\top) X)^\top \vectz(\Pi_X).
\end{aligned}
\]
Combine all terms and we will have
\begin{equation}\label{kp-Stiefel-vec}
\begin{aligned}
\frac{k_p(X,Y)}{k(X,Y)}&=C(X,Y)+\frac{1}{2} \vectz(\Pi_X)^\top (X^\top Y\otimes I_N- X^\top\otimes Y \cdot S_{N,r})\vectz(\Pi_Y) \\
&+\vectz(\mathscr{A}( \nabla^{\mathbb{R}}_Y \log k Y^\top) X)^\top \vectz(\Pi_X)+\vectz(\mathscr{A}( \nabla^{\mathbb{R}}_X \log k X^\top) Y)^\top \vectz(\Pi_Y).
\end{aligned} 
\end{equation}



\begin{theorem}[MKSDE for exponential family] Given the exponential family $p_\theta\propto\exp(\zeta(X)^\top\theta+\eta(X))$, we let
\begin{equation}
\begin{aligned}
    b(X,Y) &= \frac{1}{2}  \mathcal{Z}(X)^\top  (X^\top Y\otimes I_N- X^\top\otimes Y \cdot S_{N,r}) \vectz(\nabla_Y\eta(Y))\cdot k(X,Y)\\
    &+ \mathcal{Z}(X)^\top\vectz(\mathscr{A}( \nabla^{\mathbb{R}}_{Y} \log k Y^\top) X) \cdot k(X,Y),
    \\
    A(X,Y) &= \frac{1}{2 } \mathcal{Z}(X)^\top (X^\top Y\otimes I_N- X^\top\otimes Y \cdot S_{N,r}) \mathcal{Z}(Y)\cdot k(X,Y),
\end{aligned}
\end{equation}
where $\mathcal{Z}(X)$ is introduced in \S\ref{Grad-Mat}. Given samples $X_i\sim w$ on $\mathcal{V}_r(N)$, the MKSDE, the global minimizer of the empirical KSD in (\ref{Uw&Vw}) between the exponential family $p_\theta$ and $q$, has a closed form given below:
\begin{equation}
\begin{aligned}
\hat{\theta}^u_n&:=\min U^w_n(\theta)= - \left[\sum_{i\neq j} A(X_i,X_j)\frac{q(X_i)q(X_j)}{w(X_i)w(X_j)}\right]^{-1} \sum_{i\neq j} b(X_i,X_j)\frac{q(X_i)q(X_j)}{w(X_i)w(X_j)}\\
\hat{\theta}^v_n&:= \min V^w_n(\theta) = - \left[\sum_{i,j} A(X_i,X_j)\frac{q(X_i)q(X_j)}{w(X_i)w(X_j)}\right]^{-1} \sum_{i,j} b(X_i,X_j)\frac{q(X_i)q(X_j)}{w(X_i)w(X_j)}
\end{aligned}
\end{equation}
For the unweighted case, we just ignore the weighted ratio \(\frac{q(X_i)q(X_j)}{w(X_i)w(X_j)}\).
\end{theorem}
\begin{proof} For exponential family, we have $\Pi_X=\nabla^\mathbb{R}_X\log p=\nabla^\mathbb{R}_X(\theta^\top\zeta)+\nabla^\mathbb{R}_X\eta$, thus $\vectz(\Pi_X)= \mathcal{Z}(X)\theta+\vectz(\nabla_X\eta(X))$. We plug it into (\ref{kp-Stiefel-vec}), then we have
\[
\begin{aligned}
\frac{k_p(X,Y)}{k(X,Y)}&=C(X,Y)+\frac{1}{2} \theta^\top \mathcal{Z}(X)^\top (X^\top Y\otimes I_N- X^\top\otimes Y \cdot S_{N,r} ) \mathcal{Z}(Y)\theta \\
&+\vectz(\mathscr{A}( \nabla^{\mathbb{R}}_Y \log k Y^\top) X)^\top\mathcal{Z}(X)\theta +\vectz(\mathscr{A}( \nabla^{\mathbb{R}}_X \log k X^\top) Y)^\top \mathcal{Z}(Y) \theta\\
&+ \frac{1}{2} \vectz(\nabla_X\eta(X))^\top (X^\top Y\otimes I_N- X^\top\otimes Y \cdot S_{N,r} ) \mathcal{Z}(Y)\theta\\
&+ \frac{1}{2} \vectz(\nabla_Y\eta(Y))^\top (Y^\top X\otimes I_N- Y^\top\otimes X \cdot S_{N,r}) \mathcal{Z}(X)\theta,
\end{aligned}
\]
which is a quadratic function of $\theta$, so the weighted KSD in (\ref{Uw&Vw}), 
which is a weighted sum of $k_p$ function will remain a quadratic function of $\theta$. Therefore, the global minimizer is as shown in the theorem. Note that the first order terms combine together when summed up over $i$ and $j$.
\end{proof}




\begin{theorem}\label{Radial-Thm} Suppose $\psi:[0,+\infty)\to\mathbb{R}$ is a continuous function. Then
\begin{enumerate}
    \item The bivariate function $\kappa(x,y):=\exp(-\psi(\Vert x-y\Vert_{\mathbb{R}^d}^2))$ for $x,y\in\mathbb{R}^d$ is a kernel on $\mathbb{R}^d$ if and only if there exists a finite Borel measure $\lambda$ on $[0,+\infty)$ such that
$
\psi(t):=-\log\int_0^{+\infty} e^{-t\sigma} d\lambda(\sigma), t\geq 0.
$
Such kernel $\kappa$ is said to be a \emph{radial kernel} on $\mathbb{R}^d$.
    \item A radial kernel $\kappa$ is $C_0$-universal on $\mathbb{R}^d$ if $\lambda$ is not concentrated at $0$. 
\end{enumerate}
\end{theorem}


The next theorem \cite[Thm. 17]{micchelli2006universal}\cite[Thm. 2]{schoenberg1938metric} characterizes the radial kernels on $\mathbb{R}^d$, which are a class of kernels that satisfy our mathematical requirements perfectly and will be extensively used in 






Let $\mathcal{X}$ be a locally compact Hausdorff topological space and $C_0(\mathcal{X})$ be the space of all continuous functions on $\mathcal{X}$ that vanish at infinity.

\begin{definition}[Qualified Kernel] A separately continuous bounded kernel $\kappa$ on $\mathcal{X}$ is \emph{qualified} if for any $f\in C_0(\mathcal{X})$ and $\epsilon>0$, there exists $g\in \mathcal{H}_\kappa $ such that $\sup |f-g|<\epsilon$.
\end{definition}

Following theorem provides us with several qualified kernels  that can be easily adopted in practice.

% \begin{tcolorbox}[colback=gray!5!white,colframe=gray!75!black,title=Kernel Qualification]
\begin{theorem}\label{kernel-universal}  Suppose $\psi:M\to \mathbb{R}^{d'}$ is a smooth embedding for some $d'>d$, and suppose $\kappa$ is $C_0$-universal on $\mathbb{R}^{d'}$, then the restriction of $\kappa$ onto $M$, i.e., $\kappa|_M:=\kappa(\psi(x),\psi(x'))$ for $x,x'\in M$ is a qualified kernel on $M$.
\end{theorem}
% \end{tcolorbox}

==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Theory and Applications of Kernel Stein Discrepancy on Riemannian Manifolds}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies the kernel Stein discrepancy (KSD) on Riemannian manifolds, discusses its applications and calculates numerous specific examples, which is important because the kernel Stein method is a significantly popular method to tackle the issue of normalization on manifolds.

This paper extends our work of \red{Kernel Stein Discrepancy on Lie Groups: Theory and Applications} by generalizing the theory on Lie Groups to all Riemannian manifolds and providing the closed-form of KSDs on Homogeneous spaces. 

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{Chris Oates, Newcastle University (chris.oates@ncl.ac.uk)}
    \item \red{Bharath Sriperumbudur, Pennsylvania State University (bks18@psu.edu)}
    \item \red{Krishnakumar Balasubramanian, University of California, Davis(kbala@ucdavis.edu)}
    \item \red{Brian Kulis, Boston University(bkulis@bu.edu)}
    \item \red{Kenji Fukumizu, The Institute of Statistical Mathematics(fukumizu@ism.ac.jp)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{Michael N. Arbel, INRIA,(michael.n.arbel@gmail.com)}
    \item \red{Minh Ha Quang, RIKEN-AIP (minh.haquang@riken.jp)}
    \item \red{Ernesto De Vito, University of Genoa(ernesto.devito@unige.it)}
    \item \red{Carlo Ciliberto, University College London (c.ciliberto@ucl.ac.uk)}
    \item \red{Ronen Talmon
, Technion — Israel Institute of Technology (ronen@ee.technion.ac.il)}
\end{itemize}

Our submission has the following keywords: \red{Stein Operator}, \red{Riemannian Manifolds}, \red{Kernel Stein Discrepancy}, \red{Homogeneous Spaces}, \red{Goodness of Fit}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Xiaoda Qu (University of Florida)}\\
\red{Baba C. Vemuri (University of Florida)}

\end{document}







































